Efficient Global Point Cloud Alignment using Bayesian Nonparametric Mixtures

Point cloud alignment is a common problem in computer vision and robotics, with applications ranging from 3D object recognition to reconstruction. We propose a novel approach to the alignment problem that utilizes Bayesian nonparametrics to describe the point cloud and surface normal densities, and branch and bound (BB) optimization to recover the relative transformation. BB uses a novel, refinable, near-uniform tessellation of rotation space using 4D tetrahedra, leading to more efficient optimization compared to the common axis-angle tessellation. We provide objective function bounds for pruning given the proposed tessellation, and prove that BB converges to the optimum of the cost function along with providing its computational complexity. Finally, we empirically demonstrate the efficiency of the proposed approach as well as its robustness to real-world conditions such as missing data and partial overlap.

==> branchAndBoundRotations.tex <==
\section{Branch and Bound over the Space of Rotations}

Branch and Bound is an algorithm to efficiently search for the optimum of a
cost function over a state space. 
When searching over a continuous state space, such as the space of
rotations and translations,
%As is usual in a branch and bound algorithm, 
it needs a method to cover
the optimization space with subsets, and suitable lower and upper
bounds on the maximum objective within each subset in the cover. 
%
Efficiency is achieved by utilizing the bounds on the maximum objective
to prune areas in the state space which have a lower upper bound than
the best current lower bound. 
%
The algorithm keeps subdividing the best subset at each iteration to
keep refining the upper and lower bounds on the objective.
%When searching over a continuous state space
%%As is usual in a branch and bound algorithm, 
%we need a method to cover
%our optimization space with subsets, and suitable lower and upper
%bounds on the maximum objective within each subset in the cover. 

In the next sections, we first show how to tessellate the space of
rotations approximately uniformly on the manifold and that this
tessellation provides a suitable cover of the space. Following this
general expose we derive upper and lower bounds for our specific
objective function. We emphasize that as long as you can derive bounds
for a given objective function over the space of rotations, $\SDdim{3}$, you can use the proposed
BB approach and reap the same benefits.




==> branchAndBoundTranslation.tex <==
\section{Branch and Bound in the Space of Translations}

To obtain the optimal translation for a given rotation, we also employ
a Branch and Bound algorithm. Since the space of translations is a
bounded subspace $\mathcal{T}$ of $\mathcal{R}^3$, the tessellation is
in terms of rectangular 3D subspaces $\mathcal{T}_i$.

\section{Upper and Lower Bounds on the Translational Alignment
Objective}

A lower bound can be obtained by simply evaluating the translational
objective function at any location inside the current tessellation
cell $\mathcal{T}_i$.

We can again derive an independent component as well as a joint upper
bound for the translational alignment objective. We give describe the
bounds in the following and leave the detailed
derivations to the supplement.

\subsection{Independent Component Upper Bound}
For a given rotation $q$, an independent component upper bound is:
\begin{align}
  \max_{t\in\mathcal{T}_i} \sum_{kk'} \pi_{kk'} N(t; \Theta_{kk'}) 
  \leq \sum_{kk'} \pi_{kk'} \max_{t\in\mathcal{T}_i} N(t; \Theta_{kk'}) 
\end{align}
Where $\max_{t\in\mathcal{T}_i} N(t; \Theta_{kk'})$ is either $N(m_{kk'};
\Theta_{kk'})$ if $m_{kk'} \in \mathcal{T}_i$ or $N(t^*;
\Theta_{kk'})$, where $t^*$ is found as:
\begin{align}
  t^* &= \argmax_{t\in\mathcal{T}_i} N(t; \Theta_{kk'}) =
  \argmin_{t\in\mathcal{T}_i} \| t - m_{kk'}\|^2_{\Sigma_{kk'}}  \\
  &= \argmin_{t\in\mathcal{T}_i} t^T\Sigma_{kk'}^{-1}t -
  2t^T\Sigma_{kk'}^{-1}m_{kk'}
\end{align}
This constraint minimization problem can be solved by finding all
minima on the faces, edges and corners of $\mathcal{T}_i$ and selecting
the minimum of those.

\section{Joint Component Upper Bound}
An joint upper bound may be obtained via the log-sum-inequality:
\begin{align}
  \max_{t\in\mathcal{T}_i}& \sum_{kk'} \pi_{kk'} N(t; \Theta_{kk'}) 
  \leq C_{kk'} +
  \max_{t\in\mathcal{T}_i} \sum_{kk'}\Gamma_{kk'} \log\left( N(t;
  \Theta_{kk'}) \right) \\
  C_{kk'} &= \sum_{kk'}\Gamma_{kk'}\log \left( \pi_{kk'}\right) +
  \log(K K')
\end{align}
where 
\begin{align}
  \Gamma_{kk'} &= \left(1+ 
\sum_{jj' \neq kk'} \frac{\pi_{jj'} C_{jj'}
\exp\left\{\tfrac{1}{2} \| t_{U_i}- m_{kk'} \|_{\Sigma_{kk'}}\right\}}{\pi_{kk'}
C_{kk'} \exp\left\{\tfrac{1}{2} \| t_{L_i}-m_{jj'}\|_{\Sigma_{jj'}}
\right\} }\right)^{-1} \\
\end{align}
%
and $t_{U_i}, t_{L_i} \in \mathcal{T}_i$ are the translations farthest away from
and closest to
the respective $m_{kk'}$. 
%
With $A = \sum_{kk'}\Gamma_{kk'}\Sigma^{-1}_{kk'}$ and $b=\sum_{kk'} \Gamma_{kk'}\Sigma^{-1}_{kk'}
m_{kk'}$ the translation $t^\star\in\mathcal{T}_i$ which achieves the
upper bound can be found as
\begin{align}
  t^\star = \argmin_{t\in\mathcal{T}_i} \left( t^T A t -2 t^T b \right)
  \,.
\end{align}
Computationally, $t^\star$ can be found with the same strategy as for
finding $t^\star$ in the independent component bound.
%There are two cases: Either the minimum $t^* \in \mathcal{T}_i$ or on
%the boundaries of $\mathcal{T}_i$.
%\begin{align}
%  \deriv{\cdot}{t} &= 2A t - 2 b \\
%  \therefore t^* &= A^{-1} b
%\end{align} which is a minimum since the sum of pos definite matrices
%$A$ is pos definite again.
%So if $t^*= A^{-1} b \in \mathcal{T}_i$ we are done. Otherwise the
%minimum has to lie on once of the boundaries of $\mathcal{T}_i$ in
%which case 
%\begin{align}
%  t = t_P + E \alpha
%\end{align} where $E$ spans the 2D coordinate system on of the edge
%plane, $t_P$ is the offset of the edge plane and $\alpha = \{\alpha_0,
%\alpha_1 \}\,; 0 \leq \alpha_{0,1} \leq 1$.
%With this the minimization becomes:
%\begin{align}
%  \min_{\alpha}& \left( t_P^T A t_P + \alpha^T E^T A E \alpha - 2
%  t_P^T b - 2 \alpha^T E^T b \right) \\
%  &= \min_{\alpha} \left( \alpha^T E^T A E \alpha - 2 \alpha^T E^T b \right) \\
%  \therefore& \alpha^* = (E^T A E)^{-1} E^T b
%\end{align}
%If we found $0 \leq \alpha_{0,1} \leq 1$ then this point is a candidate
%for a minimum and will be compared against all other candidates in the
%end. We perform the same kind of analysis for all edges of
%$\mathcal{T}_i$ and also consider all corner points of the set.
%Then we choose the point of the candidate set which gives the overall
%minimum value and use it to compute the upper bound.



==> figure600Cell/figureWrapped.tex <==
\begin{wrapfigure}{r}{0.39\textwidth}
  \vspace{-0.8cm}
  \centering
  \includegraphics[width=.39\textwidth]{{./figuresSmall/Schlegel_wireframe_600-cell_vertex-centered}.png}
  \caption{A 3D projection of the
  600-cell~\cite{StellaSoft}---a 4D object 
tessellating the rotation space for the proposed branch and
bound approach to point cloud alignment.\label{fig:600cell}}
%  \vspace{-0.8cm}
\end{wrapfigure}


==> figureAngularPrecision/figure.tex <==
\begin{figure}
  \includegraphics[width=0.5\columnwidth]{{./figures/angularPrecisionVsSubdivisionLvl}.png}
  \caption{Number of subdivision levels needed for a desired angular
  precision.\label{fig:angularPrecision}}
\end{figure}


==> figureMinAngleBounds/figure.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.9\columnwidth]{{./figures/subdivisionVsMinAngle_ActualAndBound}.png}
  \caption{The actual minimal angle $\cos^{-1}\gamma$ and maximal angle $\cos^{-1}\Gamma$ angle between two
  tetrahedron vertices for
increasing refinement level, compared to the derived bounds in Lemma
\ref{lem:skew}.\label{fig:minAngleBounds}}
\end{figure}


==> figureTetrahedron/figureWithEdgeDescriotion.tex <==
\begin{figure}
  \begin{tikzpicture}
    \node (L0) at (0,0) {
      \includegraphics[width=0.3\columnwidth]{{./figures/tetrahedron_0_cropped}.png}
    };
    \node[right = 0.5ex of L0] (L1) {
      \includegraphics[width=0.3\columnwidth]{{./figures/tetrahedron_1_cropped}.png}
    };
    \node[right = 0.5ex of L1] (L2) {
      \includegraphics[width=0.3\columnwidth]{{./figures/tetrahedron_2_cropped}.png}
    };
%    \node[above = 1ex of L0] {Icosahedron};
%    \node[above = 1ex of L1] {Subdivision 1};
%    \node[above = 1ex of L2] {Subdivision 2};
  \end{tikzpicture}
  \caption{The three possible subdivision patterns of a
  tetrahedron displayed in 3D. 
  The different colors designate corner
edges (red), tie edges (green) and skew edges
(blue).\label{fig:tetrahedronSubdivision}}
\end{figure}

